Exploring the Emotional and Mental Well-Being of Individuals with Long COVID Through Twitter Analysis

The COVID-19 pandemic has led to the emergence of Long COVID, a cluster of symptoms that persist after infection. Long COVID patients may also experience mental health challenges, making it essential to understand individuals' emotional and mental well-being. This study aims to gain a deeper understanding of Long COVID individuals' emotional and mental well-being, identify the topics that most concern them, and explore potential correlations between their emotions and social media activity. Specifically, we classify tweets into four categories based on the content, detect the presence of six basic emotions, and extract prevalent topics. Our analyses reveal that negative emotions dominated throughout the study period, with two peaks during critical periods, such as the outbreak of new COVID variants. The findings of this study have implications for policy and measures for addressing the mental health challenges of individuals with Long COVID and provide a foundation for future work.

==> citation.tex <==
@article{Miao2022AnIA,
  title={An Interactive Analysis of User-reported Long COVID Symptoms using Twitter Data},
  author={Lin Miao and Mark Last and Marina Litvak},
  journal={Proceedings of the 2nd Workshop on Deriving Insights from User-Generated Text},
  year={2022}
}

@article{Callard2020HowAW,
  title={How and why patients made Long Covid},
  author={Felicity Callard and Elisa Perego},
  journal={Social Science \& Medicine (1982)},
  year={2020},
  volume={268}
}

@inproceedings{Davis2020CharacterizingLC,
  title={Characterizing Long COVID in an International Cohort: 7 Months of Symptoms and Their Impact},
  author={Hannah E. Davis and Gina S. Assaf and Lisa McCorkell and Hannah Wei and Ryan J. Low and Yochai Re’em and Signe Redfield and Jared P. Austin and Athena Akrami},
  booktitle={medRxiv},
  year={2020}
}

@article{Ballering2022PersistenceOS,
  title={Persistence of somatic symptoms after COVID-19 in the Netherlands: an observational cohort study},
  author={Aranka Vivi{\"e}nne Ballering and Sander K. R. van Zon and T. C. Olde Hartman and Judith G. M. Rosmalen},
  journal={Lancet (London, England)},
  year={2022},
  volume={400},
  pages={452 - 461}
}

@article{HoubenWilke2022TheIO,
  title={The Impact of Long COVID-19 on Mental Health: Observational 6-Month Follow-Up Study},
  author={Sarah Houben-Wilke and Yvonne M. J. Go{\"e}rtz and Jeannet M Delbressine and Anouk W. Vaes and Roy Meys and Felipe Vc Machado and Maarten van Herck and Chris Burtin and Rein Posthuma and Frits M.E. Franssen and Herman Vijlbrief and Yvonne Spies and Alex J. van ’t Hul and Martijn A. Spruit and Daisy J. A. Janssen},
  journal={JMIR Mental Health},
  year={2022},
  volume={9}
}

@article{Burton2022FactorsST,
  title={Factors shaping the mental health and well-being of people experiencing persistent COVID-19 symptoms or ‘long COVID’: qualitative study},
  author={Alexandra Burton and Henry Aughterson and Daisy Fancourt and Keir E. J. Philip},
  journal={BJPsych Open},
  year={2022},
  volume={8}
}

@article{Saha2020PsychosocialEO,
  title={Psychosocial Effects of the COVID-19 Pandemic: Large-scale Quasi-Experimental Study on Social Media},
  author={Koustuv Saha and John B Torous and Eric D. Caine and Munmun de Choudhury},
  journal={Journal of Medical Internet Research},
  year={2020},
  volume={22}
}

@article{Davis2023LongCM,
  title={Long COVID: major findings, mechanisms and recommendations},
  author={Hannah E. Davis and Lisa McCorkell and Julia Moore Vogel and Eric J. Topol},
  journal={Nature Reviews. Microbiology},
  year={2023},
  volume={21},
  pages={133 - 146}
}

@article{Proal2021LongCO,
  title={Long COVID or Post-acute Sequelae of COVID-19 (PASC): An Overview of Biological Factors That May Contribute to Persistent Symptoms},
  author={Amy D. Proal and Michael B. VanElzakker},
  journal={Frontiers in Microbiology},
  year={2021},
  volume={12}
}

@article{Haffke2022EndothelialDA,
  title={Endothelial dysfunction and altered endothelial biomarkers in patients with post-COVID-19 syndrome and chronic fatigue syndrome (ME/CFS)},
  author={Milan Haffke and Helma Freitag and Gordon Rudolf and Martina Seifert and Wolfram Doehner and Nadja Scherbakov and Leif Gunnar Hanitsch and Kirsten Wittke and Sandra Bauer and Frank Konietschke and Friedemann Paul and Judith Bellmann-Strobl and Claudia Kedor and Carmen Scheibenbogen and Franziska Sotzny},
  journal={Journal of Translational Medicine},
  year={2022},
  volume={20}
}

@article{Charfeddine2021LongC1,
  title={Long COVID 19 Syndrome: Is It Related to Microcirculation and Endothelial Dysfunction? Insights From TUN-EndCOV Study},
  author={Salma Charfeddine and Hassen Ibn hadj amor and Jihen Jdidi and Slim Torjmen and Salma Kraiem and Rania Hammami and Amine Bahloul and Nesrine Kallel and Nedia Moussa and Imen Touil and Aiman Ghrab and Jamel Elghoul and Zineb Meddeb and Yamina Thabet and Samir Kammoun and Kamel Bouslama and Sami Milouchi and Salem Ben Abdessalem and Leila Abid},
  journal={Frontiers in Cardiovascular Medicine},
  year={2021},
  volume={8}
}

@article{Pretorius2022PrevalenceOS,
  title={Prevalence of symptoms, comorbidities, fibrin amyloid microclots and platelet pathology in individuals with Long COVID/Post-Acute Sequelae of COVID-19 (PASC)},
  author={Etheresia Pretorius and Chantelle Venter and Gert Jacobus Laubscher and Maritha J. Kotze and Sunday Olukayode Oladejo and Liam R. Watson and Kanshu Rajaratnam and Bruce W. Watson and Douglas B. Kell},
  journal={Cardiovascular Diabetology},
  year={2022},
  volume={21}
}

@article{Yeoh2021GutMC,
  title={Gut microbiota composition reflects disease severity and dysfunctional immune responses in patients with COVID-19},
  author={Yun Kit Yeoh and Tao Zuo and Grace Chung Yan Lui and Fen Zhang and Qin Liu and Amy Y.L. Li and Arthur C.-K. Chung and Chun Pan Cheung and Eugene Y.K. Tso and Kitty S. C. Fung and Veronica Chan and Lowell Ling and Gavin Matthew Joynt and David Shu-cheong Hui and Kai Ming Chow and Susanna So Shan Ng and Timothy Li and Rita WY Ng and Terry Cf Yip and Grace Lai‐Hung Wong and Francis Kl Chan and Chun Kwok Wong and Paul K. S. Chan and Siew C Ng},
  journal={Gut},
  year={2021},
  volume={70},
  pages={698 - 706}
}

@article{Liu2022GutMD,
  title={Gut microbiota dynamics in a prospective cohort of patients with post-acute COVID-19 syndrome},
  author={Qin Liu and Joyce Wing Yan Mak and Qi Su and Yun Kit Yeoh and Grace Chung Yan Lui and Susanna So Shan Ng and Fen Zhang and Amy Y.L. Li and Wenqi Lu and David Shu-Cheong Hui and Paul K. S. Chan and Francis Ka Leung Chan and Siew C. Ng},
  journal={Gut},
  year={2022}
}

@article{Demko2022PostacuteSO,
  title={Post-acute sequelae of SARS-CoV-2 (PASC) impact quality of life at 6, 12 and 18 months post-infection},
  author={Zoe O Demko and Tong Yu and Smitha Mullapudi and M. G. Varela Heslin and Charmaine Dorsey and Christine B. Payton and Jeffrey A. Tornheim and Paul W Blair and S H Mehta and D. L. Thomas and YC Manabe and Annukka A R Antar and The Co-Stars Study Team},
  journal={medRxiv : the preprint server for health sciences},
  year={2022}
}

@article{Cairns2005ASR,
  title={A systematic review describing the prognosis of chronic fatigue syndrome.},
  author={Ruth Cairns and Matthew Hotopf},
  journal={Occupational medicine},
  year={2005},
  volume={55 1},
  pages={20-31}
}

@article{Taquet2021SixmonthSO,
  title={Six-month sequelae of post-vaccination SARS-CoV-2 infection: A retrospective cohort study of 10,024 breakthrough infections},
  author={Maxime Taquet and Quentin Dercon and Paul J Harrison},
  journal={Brain, Behavior, and Immunity},
  year={2021},
  volume={103},
  pages={154 - 162}
}

@article{AlAly2022LongCA,
  title={Long COVID after breakthrough SARS-CoV-2 infection},
  author={Ziyad Al‐Aly and Benjamin Bowe and Yan Xie},
  journal={Nature Medicine},
  year={2022},
  volume={28},
  pages={1461 - 1467}
}

@article{Mackey2020MachineLT,
  title={Machine Learning to Detect Self-Reporting of Symptoms, Testing Access, and Recovery Associated With COVID-19 on Twitter: Retrospective Big Data Infoveillance Study},
  author={Tim Ken Mackey and Vidya Purushothaman and Jiawei Li and Neal Shah and Matthew C. Nali and Cortni Bardier and Bryan Liang and Mingxiang Cai and Raphael E Cuomo},
  journal={JMIR Public Health and Surveillance},
  year={2020},
  volume={6}
}

@article{Banda2020LongtermPS,
  title={Long-term patient-reported symptoms of COVID-19: an analysis of social media data},
  author={Jethro Banda and Gaurav Singh and Osaid Alser and Daniel Prieto-Alhambra},
  journal={medRxiv},
  year={2020}
}

@article{Singh2020AnAO,
  title={An Analysis of Self-reported Longcovid Symptoms on Twitter},
  author={S. Manjit Singh and Chaitanya Thopi Reddy},
  journal={medRxiv},
  year={2020}
}

@article{Muri2021COVID19VH,
  title={COVID-19 Vaccine Hesitancy on Social Media: Building a Public Twitter Data Set of Antivaccine Content, Vaccine Misinformation, and Conspiracies},
  author={Goran Muri{\'c} and Yusong Wu and Emilio Ferrara},
  journal={JMIR Public Health and Surveillance},
  year={2021},
  volume={7}
}

@inproceedings{Martin2022LongCOVIDAC,
  title={\#LongCOVID affects children too: A Twitter analysis of healthcare workers sentiment and discourse about Long COVID in children and young people in the UK},
  author={Sam Martin and Macarena Chepo and Nicholas A. Deom and Ahmad Firas Khalid and Cecilia Vindrola‐Padros},
  booktitle={medRxiv},
  year={2022}
}

@article{Santarossa2021UnderstandingT,
  title={Understanding the \#longCOVID and \#longhaulers Conversation on Twitter: Multimethod Study},
  author={Sara Santarossa and Ashley Rapp and Saily Sardinas and Janine Hussein and Alex Ram{\'i}rez and Andrea E. Cassidy-Bushrow and Philip Cheng and Eunice Yu},
  journal={Jmir Infodemiology},
  year={2021},
  volume={2}
}

@article{Chen2020TrackingSM,
  title={Tracking Social Media Discourse About the COVID-19 Pandemic: Development of a Public Coronavirus Twitter Data Set},
  author={Emily Chen and Kristina Lerman and Emilio Ferrara},
  journal={JMIR Public Health and Surveillance},
  year={2020},
  volume={6}
}

@article{Awoyemi2022TwitterSA,
  title={Twitter Sentiment Analysis of Long COVID Syndrome},
  author={Toluwalase Awoyemi and Ujunwa Ebili and Abiola Olusanya and Kayode E Ogunniyi and Adedolapo V Adejumo},
  journal={Cureus},
  year={2022},
  volume={14}
}

@article{TurnerMcGrievy2015TweetFH,
  title={Tweet for health: using an online social network to examine temporal trends in weight loss-related posts},
  author={Gabrielle M. Turner-McGrievy and Michael W. Beets},
  journal={Translational Behavioral Medicine},
  year={2015},
  volume={5},
  pages={160-166}
}

@article{Harris2014ArePH,
  title={Are Public Health Organizations Tweeting to the Choir? Understanding Local Health Department Twitter Followership},
  author={Jenine K. Harris and Bechara Choucair and Ryan C. Maier and Nina Jolani and Jay M. Bernhardt},
  journal={Journal of Medical Internet Research},
  year={2014},
  volume={16}
}

@article{Blei2001LatentDA,
  title={Latent Dirichlet Allocation},
  author={David M. Blei and A. Ng and Michael I. Jordan},
  journal={J. Mach. Learn. Res.},
  year={2001},
  volume={3},
  pages={993-1022}
}

@article{Culmer2021ExaminingLA,
  title={Examining LDA2Vec and Tweet Pooling for Topic Modeling on Twitter Data},
  author={Kristofferson Culmer and Jeffrey K. Uhlmann},
  journal={WSEAS TRANSACTIONS ON INFORMATION SCIENCE AND APPLICATIONS},
  year={2021}
}

@article{Koshute2021RecommendingTS,
  title={Recommending Training Set Sizes for Classification},
  author={Phillip T. Koshute and Jared Zook and Ian McCulloh},
  journal={ArXiv},
  year={2021},
  volume={abs/2102.09382}
}

@inproceedings{Gregory2020ATA,
  title={A Transformer Approach to Contextual Sarcasm Detection in Twitter},
  author={Hunter Gregory and Steven Li and Pouya Mohammadi and Natalie Tarn and Rachel Lea Draelos and Cynthia Rudin},
  booktitle={FIGLANG},
  year={2020}
}

@article{Liu2019RoBERTaAR,
  title={RoBERTa: A Robustly Optimized BERT Pretraining Approach},
  author={Yinhan Liu and Myle Ott and Naman Goyal and Jingfei Du and Mandar Joshi and Danqi Chen and Omer Levy and Mike Lewis and Luke Zettlemoyer and Veselin Stoyanov},
  journal={ArXiv},
  year={2019},
  volume={abs/1907.11692}
}

@article{Barbieri2020TweetEvalUB,
  title={TweetEval: Unified Benchmark and Comparative Evaluation for Tweet Classification},
  author={Francesco Barbieri and Jos{\'e} Camacho-Collados and Leonardo Neves and Luis Espinosa-Anke},
  journal={ArXiv},
  year={2020},
  volume={abs/2010.12421}
}

@article{Butt2021WhatGO,
  title={What goes on inside rumour and non-rumour tweets and their reactions: A Psycholinguistic Analyses},
  author={Sabur Butt and Shakshi Sharma and Rajesh Sharma and Grigori Sidorov and Alexander F. Gelbukh},
  journal={Comput. Hum. Behav.},
  year={2021},
  volume={135},
  pages={107345}
}

@article{Rozado2022LongitudinalAO,
  title={Longitudinal analysis of sentiment and emotion in news media headlines using automated labelling with Transformer language models},
  author={David Rozado and Ruth Hughes and Jamin B. Halberstadt},
  journal={PLoS ONE},
  year={2022},
  volume={17}
}

@article{Kuang2022MusictoTextSG,
  title={Music-to-Text Synaesthesia: Generating Descriptive Text from Music Recordings},
  author={Zhihuan Kuang and Shi Zong and Jianbing Zhang and Jiajun Chen and Hongfu Liu},
  journal={ArXiv},
  year={2022},
  volume={abs/2210.00434}
}

@article{Ehrenreich2007TheRO,
  title={The Role of Emotion in Psychological Therapy.},
  author={Jill T. Ehrenreich and Christopher P. Fairholme and Brian A. Buzzella and Kristen K Ellard and David H. Barlow},
  journal={Clinical psychology : a publication of the Division of Clinical Psychology of the American Psychological Association},
  year={2007},
  volume={14 4},
  pages={
          422-428
        }
}

@inproceedings{AlHameed2022SpearmansCC,
  title={Spearman’s correlation coefficient in statistical analysis},
  author={Khawla Ali Abd Al-Hameed},
  year={2022}
}

@article{Miot2018CorrelationAI,
  title={Correlation analysis in clinical and experimental studies},
  author={H{\'e}lio Amante Miot},
  journal={Jornal Vascular Brasileiro},
  year={2018},
  volume={17},
  pages={275 - 279}
}

@book{iversen2012statistics,
  title={Statistics: The conceptual approach},
  author={Iversen, Gudmund R and Gergen, Mary},
  year={2012},
  publisher={Springer Science \& Business Media}
}

@inproceedings{Hoffman2010OnlineLF,
  title={Online Learning for Latent Dirichlet Allocation},
  author={Matthew D. Hoffman and David M. Blei and Francis R. Bach},
  booktitle={NIPS},
  year={2010}
}

@article{Ekman1992AnAF,
  title={An argument for basic emotions},
  author={Paul Ekman},
  journal={Cognition \& Emotion},
  year={1992},
  volume={6},
  pages={169-200}
}
